Harnessing Integrated CPU-GPU System Memory for HPC: a first look into Grace Hopper

Memory management across discrete CPU and GPU physical memory is traditionally achieved through explicit GPU allocations and data copy or unified virtual memory. The Grace Hopper Superchip, for the first time, supports an integrated CPU-GPU system page table, hardware-level addressing of system allocated memory, and cache-coherent NVLink-C2C interconnect, bringing an alternative solution for enabling a Unified Memory system. In this work, we provide the first in-depth study of the system memory management on the Grace Hopper Superchip, in both in-memory and memory oversubscription scenarios. We provide a suite of six representative applications, including the Qiskit quantum computing simulator, using system memory and managed memory. Using our memory utilization profiler and hardware counters, we quantify and characterize the impact of the integrated CPU-GPU system page table on GPU applications. Our study focuses on first-touch policy, page table entry initialization, page sizes, and page migration. We identify practical optimization strategies for different access patterns. Our results show that as a new solution for unified memory, the system-allocated memory can benefit most use cases with minimal porting efforts.

==> GNN.tex <==
\section{Case Study II: Graph Neural Network}

GNN In-memory

GNN Out-of-memory


==> data-cacheline.tex <==
\section{Fine-grained Cacheline Access}
One of effect of seeing high performance of sysmalloc and only using CPU-side memory for regular access pattern, come from the cache coherence. Fine-grained cachelines are fetched from CPU side and cached in GPU's caches.

\subsection{Traffic Amplification} over the CPU-GPU interconnect
compare between system-allocated memory and managed memory. 

Observation: L2 through = Sum of (), UM bottlenecked by C2C link, sysmalloc has higher .

Takeaway: high throughput NvlinkC2C and cacheline access can sustain high performance, if not optimized the first touch and page placement properly, applications may end up with remote traffic instead of local traffic to device memory.

Optimization: we proactively prefetch pages after the first-touch to GPU. Show reduction in Nvlink-C2C traffic and increased local memory traffic.

\subsection{Cache Coherence Traffic}
we observe high write back traffic.

huge write traffic and coherence ,  BFS is read-only . 

Qiskit has a long initialization phase due to GPU writes to mallocatoin. 

Qiskit: initialization on GPU huge write traffic, computation phase: repeated shots 10 shorts.

Takeaway: 



==> discussion.tex <==
\section{Discussions and Takeaways}

Obs 1: Cache coherence in system maanaged 

application should have slower version in UM than sysmalloc: all Rodina except SRAD is faster. Qubits 22 and above UM is increasingly faster than sysmalloc. (Initialization phase is slower, and compute phases are similar)

Future direction: 



